CNN-Aided Factor Graphs with Estimated Mutual Information Features for Seizure Detection

We propose a convolutional neural network (CNN) aided factor graphs assisted by mutual information features estimated by a neural network for seizure detection. Specifically, we use neural mutual information estimation to evaluate the correlation between different electroencephalogram (EEG) channels as features. We then use a 1D-CNN to extract extra features from the EEG signals and use both features to estimate the probability of a seizure event.~Finally, learned factor graphs are employed to capture the temporal correlation in the signal. Both sets of features from the neural mutual estimation and the 1D-CNN are used to learn the factor nodes. We show that the proposed method achieves state-of-the-art performance using 6-fold leave-four-patients-out cross-validation.

==> Test.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% File:     spconf.sty          (LaTeX Document style option "spconf")
%
% Usage:    \documentclass{article}
%           \usepackage{spconf}
%
%           Or for LaTeX 2.09:
% Usage:    \documentstyle[...,spconf,...]{article}
%
% Purpose:
%
% Style file for Signal Processing Society Conferences (ICASSP, ICIP).
% Features:
%    - correct page size (175mm x 226mm)
%    - twocolumn format
%    - boldfaced, numbered, and centered section headings
%    - correct subsection and subsubsection headings
%    - use \title{xx} for title, will be typeset all uppercase
%    - use \name{xx} for author name(s) only, will be typeset in italics
%    - use \address{xx} for one address of all authors
%    - use \twoauthors{author1}{address1}{author2}{address2}
%         for two (or more) authors with two separate addresses
%    - note: no need for \author nor \date
%    - optional: can use \thanks{xx} within \name or \twoauthors,
%         asterisk is not printed after name nor in footnote
%    - optional: can use \sthanks{xx} after each name within \name or
%         \twoauthors if different thanks for each author,
%         footnote symbol will appear for each name and footnote
%    - optional: use \ninept to typeset text in 9 pt; default is 10pt.
%
% Example of use for one or more authors at a common address and
%    common support. For distinct support acknowledgments,
%    use \sthanks{xx} after each name.
%
%                 \documentclass{article}
%                 \usepackage{spconf}
%                 \title{Title of the paper}
%                 \name{George P. Burdell and John Q. Professor
%                       \thanks{This work was supported by...}}
%                 \address{Common address, department \\
%                          City, etc \\
%                          optional e-mail address}
%
%                 \begin{document}
%  OPTIONAL -->   \ninept            <-- OPTIONAL, for nine pt only
%                 \maketitle
%                 \begin{abstract}
%                 This is the abstract for my paper.
%                 \end{abstract}
%                         .
%                 Insert text of paper
%                         .
%                 \end{document}
%
% Example of use for two authors at two distinct addresses with only
%    one support acknowledgment. For distinct support acknowledgments,
%    use \sthanks{xx} after each name.
%
%                 \documentclass{article}
%                 \usepackage{spconf}
%                 \title{Title of the paper}
%                 \twoauthors{John Doe
%                       \thanks{This work was supported by...}}
%                            {Doe's address, department \\
%                             City, etc \\
%                             optional e-mail address}
%                            {Judy Smith}
%                            {Smith's address, department \\
%                             City, etc \\
%                             optional e-mail address}
%
%                 \begin{document}
%  OPTIONAL -->   \ninept            <-- OPTIONAL, for nine pt only
%                 \maketitle
%                 \begin{abstract}
%                 This is the abstract for my paper.
%                 \end{abstract}
%                         .
%                 Insert text of paper
%                         .
%                 \end{document}
%
% Preprint Option (Only for preprints, not for submissions!):
%    - can create a preprint titlepage footer by using the
%         "preprint" option with the \usepackage{spconf} command
%    - use \copyrightnotice{\copyright xx} for copyright information
%    - use \toappear{To appear in xx} for publication name
% Example of preprint use:
%
%                 \documentclass{article}
%                 \usepackage[preprint]{spconf}
%                         .
%                 \copyrightnotice{\copyright\ IEEE 2000}
%                 \toappear{To appear in {\it Proc.\ ICASSP2000,
%                    June 05-09, 2000, Istanbul, Turkey}}
%
%
% PLEASE REPORT ANY BUGS
%
% Author:  Stephen Martucci  -- stephen.martucci@ieee.org
%
% Date:    3 May 2000
%
% Updated: Lance Cotton, Ulf-Dietrich Braumann, 11 May 2006
% Change:  Added keywords/Index Terms section
% Change:  Added \emergencystretch=11pt, Lance Cotton, 26-Sept-2007
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% These commands change default text fonts to the scalable PostScript
% fonts Times, Helvetica, and Courier. However, they do not change
% the default math fonts. After conversion to PDF, text will look good
% at any scale but math symbols and equations may not.
% If instead you use the PostScript Type 1 implementation of the
% Computer Modern fonts from the American Mathematical Society, which
% will make all fonts (text and math) scalable, comment out the
% following three lines. Those fonts use the same metrics as the Knuth
% Computer Modern fonts and therefore no font redefinition is needed.
\renewcommand{\sfdefault}{phv}
\renewcommand{\rmdefault}{ptm}
\renewcommand{\ttdefault}{pcr}

%\oddsidemargin  -0.31in
%\evensidemargin -0.31in
\oddsidemargin  -6.2truemm
\evensidemargin -6.2truemm

\topmargin 0truept
\headheight 0truept
\headsep 0truept
%\footheight 0truept
%\footskip 0truept
\textheight 229truemm
\textwidth 178truemm

\twocolumn
\columnsep 6truemm
\pagestyle{empty}

\emergencystretch=11pt

\def\ninept{\def\baselinestretch{.95}\let\normalsize\small\normalsize}

\def\maketitle{\par
 \begingroup
 \def\thefootnote{}
 \def\@makefnmark{\hbox
 {$^{\@thefnmark}$\hss}}
 \if@twocolumn
 \twocolumn[\@maketitle]
 \else \newpage
 \global\@topnum\z@ \@maketitle \fi\@thanks
 \endgroup
 \setcounter{footnote}{0}
 \let\maketitle\relax
 \let\@maketitle\relax
 \gdef\thefootnote{\arabic{footnote}}\gdef\@@savethanks{}%
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}

\def\@maketitle{\newpage
 \null
 \vskip 2em \begin{center}
 {\large \bf \@title \par} \vskip 1.5em {\large \lineskip .5em
\begin{tabular}[t]{c}\@name \\ \@address
 \end{tabular}\par} \end{center}
 \par
 \vskip 1.5em}

\def\title#1{\gdef\@title{\uppercase{#1}}}
\def\name#1{\gdef\@name{{\em #1}\\}}
\def\address#1{\gdef\@address{#1}}
\gdef\@title{\uppercase{title of paper}}
\gdef\@name{{\em Name of author}\\}
\gdef\@address{Address - Line 1 \\
               Address - Line 2 \\
               Address - Line 3}

\let\@@savethanks\thanks
\def\thanks#1{\gdef\thefootnote{}\@@savethanks{#1}}
\def\sthanks#1{\gdef\thefootnote{\fnsymbol{footnote}}\@@savethanks{#1}}

\def\twoauthors#1#2#3#4{\gdef\@address{}
   \gdef\@name{\begin{tabular}{@{}c@{}}
        {\em #1} \\ \\
        #2\relax
   \end{tabular}\hskip 1in\begin{tabular}{@{}c@{}}
        {\em #3} \\ \\
        #4\relax
\end{tabular}}}

\def\@sect#1#2#3#4#5#6[#7]#8{
   \refstepcounter{#1}\edef\@svsec{\csname the#1\endcsname.\hskip 0.6em}
       \begingroup \ifnum #2=1\bf\centering
          {\interlinepenalty \@M
             \@svsec\uppercase{#8}\par}\else\ifnum #2=2\bf
          \noindent{\interlinepenalty \@M \@svsec #8\par}\else\it
          \noindent{\interlinepenalty \@M
             \@svsec #8\par}\fi\fi\endgroup
       \csname #1mark\endcsname{#7}\addcontentsline
         {toc}{#1}{\protect\numberline{\csname the#1\endcsname} #7}
     \@tempskipa #5\relax
     \@xsect{\@tempskipa}}

\def\abstract{\begin{center}
{\bf ABSTRACT\vspace{-.5em}\vspace{0pt}}
\end{center}}
\def\endabstract{\par}

% Keyword section, added by Lance Cotton, adapted from IEEEtrans, corrected by Ulf-Dietrich Braumann
\def\keywords{\vspace{.5em}
{\bfseries\textit{Index Terms}---\,\relax%
}}
\def\endkeywords{\par} 

\def\copyrightnotice#1{\gdef\@copyrightnotice{#1}}
\let\@copyrightnotice\relax
\def\toappear#1{\gdef\@toappear{#1}}\let\@toappear\relax

\newif\if@preprint\@preprintfalse
\@namedef{ds@preprint}{\global\@preprinttrue}
\@options
\def\ps@preprint{\def\mypage{}\let\@mkboth\@gobbletwo\def\@oddhead{}
  \def\@oddfoot{\rlap{\@toappear}\hfil\mypage\hfil
    \llap{\@copyrightnotice}
    \gdef\mypage{\thepage}\gdef\@toappear{}\gdef\@copyrightnotice{}}}

\if@preprint\ps@preprint
\else\ps@empty\flushbottom\fi

\def\thebibliography#1{\section{References}\list
 {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
 \advance\leftmargin\labelsep
 \usecounter{enumi}}
 \def\newblock{\hskip .11em plus .33em minus .07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist

\long\def\@makecaption#1#2{
 \vskip 10pt
 \setbox\@tempboxa\hbox{#1. #2}
 \ifdim \wd\@tempboxa >\hsize #1. #2\par \else \hbox
to\hsize{\hfil\box\@tempboxa\hfil}
 \fi}

\def\fnum@figure{{\bf Fig.\ \thefigure}}
\def\fnum@table{{\bf Table \thetable}}

\flushbottom

%%%% EOF

==> preamble.tex <==

\newcommand{\myVec}[1]{{\boldsymbol{#1}}}
\newcommand{\myMat}[1]{{\boldsymbol{#1}}}
\newcommand{\mySet}[1]{\mathcal{#1}}
% Here is a list of commands which I should consider using in the manuscript:
\newcommand{\E}{\mathds{E}}		 			% Stochastic expectation
\newcommand{\myI}{{\myMat{I}}}			 		% Identity matrix
\newcommand{\myX}{{\myVec{x}}}			 		% Obsevations
\newcommand{\myY}{\myVec{y}}
\newcommand{\myWeights}{\myVec{w}}
\newcommand{\myWeightsV}{\bar{\myWeights}}
\newcommand{\myUpdate}{\myVec{h}}
\newcommand{\myUpdateV}{\bar{\myVec{h}}}
\newcommand{\myGlobalModel}{\tilde{\myWeights}} 
\newcommand{\myGlobalModelV}{\bar{\myWeights}} 
\newcommand{\Nusers}{K}
\newcommand{\Ntraining}{n}
\newcommand{\Rate}{R}
\newcommand{\Nlattice}{L}
\newcommand{\Npoints}{M}
\newcommand{\GenMat}{\myMat{G}}
\newcommand{\Partition}{\mySet{P}_0}
\newcommand{\Desired}{^{\rm des}}
\newcommand{\Opt}{^{\rm o}}
\newcommand{\NoCite}{\textcolor{red}{[CITE]}}
\newcommand{\Verify}{\footnote{\textcolor{red}{TODO NIR VERIFY} }}
\newcommand{\FwdMsg}[2]{\overrightarrow{\mu}_{#2}}
\newcommand{\BwdMsg}[2]{\overleftarrow{\mu}_{#2}}%{\mu_{#1 \rightarrow #2}}

\newcommand{\Pdf}[1]{P_{ { #1}} }
\newcommand{\PdfEst}[1]{\hat{P}_{ { #1}} }
\newcommand{\Mem}{l}			 			% observations length
\newcommand{\Blklen}{t}			 			% observations length
\newcommand{\Codlen}{b}			 			% observations length
\newcommand{\Blkset}{\mySet{T}}
\newcommand{\CnstSize}{m}	
\newcommand{\NonStatBlk}{t_b}

\newcommand{\lenX}{n}			 			% observations length
\newcommand{\lenS}{k}			 			% Parameters length
\newcommand{\lenSset}{\mySet{K}}			 			% Parameters length
\newcommand{\lenXset}{\mySet{N}}			 			% Parameters length
\newcommand{\Quan}[2]{Q_{#1}^{#2}}
\newcommand{\myC}{{\myVec{c}}}			 		% Obsevations
\newcommand{\CovMat}[1]{\myMat{\Sigma}_{#1}}			% covariance matrix
\newcommand{\eig}[1]{\lambda_{#1}}			% covariance matrix 



\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Comment}
\newtheorem{example}{Example}



\acrodef{adc}[ADC]{analog-to-digital convertor}
\acrodef{cs}[CS]{compressed sensing}
\acrodef{bp}[BP]{belief propagation}
\acrodef{sp}[SP]{sum-product}
\acrodef{dtft}[DTFT]{discrete-time Fourier transform}
\acrodef{dnn}[DNN]{deep neural network} 
\acrodef{csi}[CSI]{channel state information}
\acrodef{map}[MAP]{maximum a-posteriori probability}
\acrodef{snr}[SNR]{signal-to-noise ratio}
\acrodef{bs}[BS]{base station} 
\acrodef{em}[EM]{expectation maximization} 
\acrodef{iot}[IOT]{Interent of Things}
\acrodef{mimo}[MIMO]{multiple-input multiple-output}
\acrodef{mse}[MSE]{mean-squared error}
\acrodef{pdf}[PDF]{probability density function}
\acrodef{rv}[RV]{random variable}
\acrodef{fec}[FEC]{forward error correction} 
\acrodef{lti}[LTI]{linear time-invariant}
\acrodef{wss}[WSS]{wide-sense stationary}
\acrodef{psd}[PSD]{power spectral density}
\acrodef{ser}[SER]{symbol error rate} 
\acrodef{ber}[BER]{bit error rate} 
\acrodef{sgd}[SGD]{stochastic gradient descent} 
\acrodef{isi}[ISI]{intersymbol interference}  
\acrodef{awgn}[AWGN]{additive white Gaussian noise} 
\acrodef{ut}[UT]{user terminal}  
\acrodef{ml}[ML]{machine learning}  
\acrodef{rnn}[RNN]{recurrent neural network}
\acrodef{sbrnn}[SBRNN]{sliding bidirectional \ac{rnn}}
\acrodef{bpsk}[BPSK]{binary phase shift keying}
\acrodef{rs}[RS]{Reed-Solomon}
\acrodef{crc}[CRC]{cyclic redundency check}
\acrodef{fc}[FC]{fully-connected}
\acrodef{hmm}[HMM]{hidden Markov model}
\acrodef{loo}[LOO]{leave-one-out}
